Enhancements to ACL2 in Versions 6.2, 6.3, and 6.4

We report on improvements to ACL2 made since the 2013 ACL2 Workshop.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{F. Verbeek and J. Schmaltz (Eds.): ACL2 Workshop 2014 (ACL2'14).\\
EPTCS 152, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.152.1}{10.4204/EPTCS.152.1}}
\pdfoutput=1

